Through the Lens of Split Vote: Exploring Disagreement, Difficulty and Calibration in Legal Case Outcome Classification

In legal decisions, split votes (SV) occur when judges cannot reach a unanimous decision, posing a difficulty for lawyers who must navigate diverse legal arguments and opinions. In high-stakes domains, understanding the alignment of perceived difficulty between humans and AI systems is crucial to build trust. However, existing NLP calibration methods focus on a classifier's awareness of predictive performance, measured against the human majority class, overlooking inherent human label variation (HLV). This paper explores split votes as naturally observable human disagreement and value pluralism. We collect judges' vote distributions from the European Court of Human Rights (ECHR), and present SV-ECHR, a case outcome classification (COC) dataset with SV information. We build a taxonomy of disagreement with SV-specific subcategories. We further assess the alignment of perceived difficulty between models and humans, as well as confidence- and human-calibration of COC models. We observe limited alignment with the judge vote distribution. To our knowledge, this is the first systematic exploration of calibration to human judgements in legal NLP. Our study underscores the necessity for further research on measuring and enhancing model calibration considering HLV in legal decision tasks.

==> table/depre_calibraton_results.tex <==

\resizebox{0.98\textwidth}{!}{
% Please add the following required packages to your document preamble:

% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{tabular}{|l|cclcclrr|}
\hline
 & \multicolumn{1}{c|}{\textbf{BERT}} & \multicolumn{1}{c|}{\textbf{BERT\_TS}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}BERT\\ \_softmax\end{tabular}}} & \multicolumn{1}{c|}{\textbf{LegalBERT}} & \multicolumn{1}{c|}{\textbf{LegalBERT\_TS}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}LegalBERT\\ \_softmax\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Oracle \\ Human\end{tabular}}} & \multicolumn{1}{l|}{\textbf{Random}} \\ \hline
 & \multicolumn{8}{c|}{\textbf{Classification}} \\ \hline
Hard-macro F1 & \multicolumn{1}{c|}{64.46 ± 3.79} & \multicolumn{1}{c|}{64.46 ± 3.79} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{68.02 ± 1.29}} & \multicolumn{1}{c|}{68.02 ± 1.29} & \multicolumn{1}{l|}{} & \multicolumn{1}{r|}{1} & \multicolumn{1}{c|}{44.96} \\ \hline
 & \multicolumn{8}{c|}{\textbf{Confidence Calibration}} \\ \hline
ECE & \multicolumn{1}{c|}{21.10 ± 4.14} & \multicolumn{1}{c|}{{\ul 2.66 ± 1.57}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{23.75 ± 1.08} & \multicolumn{1}{c|}{\textbf{2.25 ± 0.77}} & \multicolumn{1}{l|}{} & \multicolumn{1}{r|}{29.32} & 15.35 \\ \hline
ACE & \multicolumn{1}{c|}{22.26 ± 7.17} & \multicolumn{1}{c|}{13.88 ± 5.12} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{24.27 ± 3.66} & \multicolumn{1}{c|}{{\ul 13.23 ± 3.43}} & \multicolumn{1}{l|}{} & \multicolumn{1}{r|}{\textbf{2.45}} & 21.39 \\ \hline
 & \multicolumn{8}{c|}{\textbf{Human Calibration}} \\ \hline
EntCE & \multicolumn{1}{c|}{{\ul 25.21 ± 10.48}} & \multicolumn{1}{c|}{55.76 ± 1.21} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{17.84 ± 1.99}} & \multicolumn{1}{c|}{55.99 ± 1.71} & \multicolumn{1}{l|}{} & \multicolumn{1}{r|}{0} & 44.75 \\ \hline
DistCE & \multicolumn{1}{c|}{{\ul 29.15 ± 2.20}} & \multicolumn{1}{c|}{37.39 ± 0.95} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{26.23 ± 1.00}} & \multicolumn{1}{c|}{36.75 ± 1.13} & \multicolumn{1}{l|}{} & \multicolumn{1}{r|}{0} & 50.34 \\ \hline
\end{tabular}
}

% }




==> table/difficulty_sv.tex <==
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{|l|cc|cc|cc|ccc|cc|}
\hline
 & \multicolumn{2}{c|}{\textbf{case\_count}} & \multicolumn{2}{c|}{\textbf{mac-f1}} & \multicolumn{2}{c|}{\textbf{mic-f1}} & \multicolumn{3}{c|}{\textbf{avg pvi}} & \multicolumn{2}{c|}{\% violaton cases} \\ \hline
 & \multicolumn{1}{c|}{SV} & all & \multicolumn{1}{c|}{SV} & all & \multicolumn{1}{c|}{SV} & all & \multicolumn{1}{c|}{SV} & \multicolumn{1}{c|}{all} & p-value & \multicolumn{1}{c|}{SV} & all \\ \hline
BERT & \multicolumn{1}{c|}{\multirow{112}} & \multirow{1575} & \multicolumn{1}{c|}{45.6 ± 1.71} & 67.1 ± 1.04 & \multicolumn{1}{c|}{54.77 ± 2.02} & 74.4 ± 0.1 & \multicolumn{1}{c|}{0.06} & \multicolumn{1}{c|}{0.94} & 0.002 & \multicolumn{1}{c|}{\multirow{0.6}} & \multirow{0.7} \\ \cline{1-1} \cline{4-10}
LegalBERT & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{49.37 ± 5.66} & 67.5 ± 0.95 & \multicolumn{1}{c|}{59.53 ± 3.69} & 75.13 ± 0.31 & \multicolumn{1}{c|}{-0.098} & \multicolumn{1}{c|}{0.772} & 0.007 & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}

}

==> table/difficulty_vio.tex <==
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{|l|cc|cc|cc|ccc|cc|}
\hline
 & \multicolumn{2}{c|}{\textbf{case\_count}} & \multicolumn{2}{c|}{\textbf{mac-f1}} & \multicolumn{2}{c|}{\textbf{mic-f1}} & \multicolumn{3}{c|}{\textbf{avg pvi}} & \multicolumn{2}{c|}{\% SV cases} \\ \hline
 & \multicolumn{1}{c|}{non-vio} & vio & \multicolumn{1}{c|}{non-vio} & vio & \multicolumn{1}{c|}{non-vio} & vio & \multicolumn{1}{c|}{non-vio} & \multicolumn{1}{c|}{vio} & p-value & \multicolumn{1}{c|}{non-vio} & vio \\ \hline
BERT & \multicolumn{1}{c|}{\multirow{486}} & \multirow{1089} & \multicolumn{1}{c|}{30.73 ± 1.97} & 46.77 ± 0.49 & \multicolumn{1}{c|}{44.4 ± 4.18} & 87.83 ± 1.78 & \multicolumn{1}{c|}{-2.19} & \multicolumn{1}{c|}{2.01} & 1e-142 & \multicolumn{1}{c|}{\multirow{0.09}} & \multirow{0.06} \\ \cline{1-1} \cline{4-10}
LegalBERT & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{30.2 ± 1.77} & 47.17 ± 0.5 & \multicolumn{1}{c|}{43.33 ± 3.66} & 89.33 ± 1.7 & \multicolumn{1}{c|}{-1.92} & \multicolumn{1}{c|}{2.13} & 2e-190 & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}
}

==> table/f1s.tex <==
\resizebox{0.95\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{tabular}{|l|c|cc|cc|cc|c|}
\hline
\multicolumn{1}{|c|}{\textbf{BERT}} & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{mac}} & \multicolumn{2}{c|}{\textbf{mic}} & \multicolumn{2}{c|}{\textbf{hm}} & \multicolumn{1}{l|}{\textbf{}} \\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{original} & soft & \multicolumn{1}{c|}{original} & soft & \multicolumn{1}{c|}{original} & soft & count \\ \hline
test & \textbf{cases w/ SV} & \multicolumn{1}{c|}{51.37 ± 7.92} & \textbf{55.8 ± 2.43} & \multicolumn{1}{c|}{53.13 ± 5.99} & \textbf{55.9 ± 0.98} & \multicolumn{1}{c|}{\textit{\textbf{47.9 ± 5.01}}} & 45.23 ± 3.25 & 159 \\ \hline
 & \textbf{all} & \multicolumn{1}{c|}{65.53 ± 6.2} & \textbf{71.27 ± 1.4} & \multicolumn{1}{c|}{72.3 ± 4.1} & \textbf{77.03 ± 0.67} & \multicolumn{1}{c|}{\textit{\textbf{64.23 ± 3.48}}} & 63.7 ± 1.47 & 1575 \\ \hline
 
% dev & \textbf{cases w/ SV} & \multicolumn{1}{c|}{46.1 ± 6.24} & \textbf{54.33 ± 1.1} & \multicolumn{1}{c|}{54.03 ± 6.11} & \textbf{64.6 ± 3.48} & \multicolumn{1}{c|}{50.1 ± 3.7} & \textbf{51.6 ± 1.99} & 178 \\ \hline
 % & \textbf{all} & \multicolumn{1}{c|}{67.23 ± 7.0} & \textbf{74.33 ± 1.0} & \multicolumn{1}{c|}{72.37 ± 5.01} & \textbf{78.83 ± 1.27} & \multicolumn{1}{c|}{66.5 ± 2.19} & \textbf{67.6 ± 0.56} & 1516 \\ \hline
 
\textbf{LegalBERT} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
test & \textbf{cases w/ SV} & \multicolumn{1}{r|}{\textbf{59.23 ± 3.98}} & \multicolumn{1}{r|}{56.37 ± 2.61} & \multicolumn{1}{r|}{58.93 ± 1.4} & \multicolumn{1}{r|}{\textbf{59.47 ± 2.95}} & \multicolumn{1}{r|}{\textbf{59.33 ± 3.93}} & \multicolumn{1}{r|}{52.27 ± 4.47} & 159 \\ \hline
 & \textbf{all} & \multicolumn{1}{r|}{68.77 ± 1.16} & \multicolumn{1}{r|}{\textbf{70.53 ± 1.07}} & \multicolumn{1}{r|}{73.57 ± 0.6} & \multicolumn{1}{r|}{\textbf{77.1 ± 0.46}} & \multicolumn{1}{r|}{\textbf{68.03 ± 1.29}} & \multicolumn{1}{r|}{65.17 ± 0.8} & 1575 \\ \hline
 
% dev & \textbf{cases w/ SV} & \multicolumn{1}{r|}{45.83 ± 3.86} & \multicolumn{1}{r|}{\textbf{51.87 ± 1.39}} & \multicolumn{1}{r|}{53.77 ± 3.95} & \multicolumn{1}{r|}{\textbf{62.07 ± 1.15}} & \multicolumn{1}{r|}{50.37 ± 3.49} & \multicolumn{1}{r|}{\textbf{52.43 ± 4.4}} & 178 \\ \hline
%  & \textbf{all} & \multicolumn{1}{r|}{71.6 ± 1.61} & \multicolumn{1}{r|}{\textbf{73.5 ± 0.44}} & \multicolumn{1}{r|}{74.1 ± 1.04} & \multicolumn{1}{r|}{\textbf{78.1 ± 0.36}} & \multicolumn{1}{r|}{68.3 ± 0.95} & \multicolumn{1}{r|}{\textbf{68.3 ± 0.66}} & 1516 \\ \hline
\end{tabular}

}


==> table/f1s_app.tex <==
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{|l|c|cc|cc|cc|c|}
\hline
\multicolumn{1}{|c|}{BERT} & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{mac}}} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{mic}}} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{hm}}} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|c|}{Test} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{normal} & soft & \multicolumn{1}{c|}{normal} & soft & \multicolumn{1}{c|}{normal} & soft & count \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/o SV}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 66.83 ± 6.35}} & {\color[HTML]{3B3B3B} \textbf{72.87 ± 1.8}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 74.33 ± 4.01}} & {\color[HTML]{3B3B3B} \textbf{79.27 ± 0.61}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} \textit{\textbf{65.9 ± 3.41}}}} & {\color[HTML]{3B3B3B} 65.73 ± 1.07} & {\color[HTML]{3B3B3B} \textbf{1416}} \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/ SV}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 51.37 ± 7.92}} & {\color[HTML]{3B3B3B} \textbf{55.8 ± 2.43}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 53.13 ± 5.99}} & {\color[HTML]{3B3B3B} \textbf{55.9 ± 0.98}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} \textit{\textbf{47.9 ± 5.01}}}} & {\color[HTML]{3B3B3B} 45.23 ± 3.25} & {\color[HTML]{3B3B3B} 159} \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{all}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 65.53 ± 6.2}} & {\color[HTML]{3B3B3B} \textbf{71.27 ± 1.4}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 72.3 ± 4.1}} & {\color[HTML]{3B3B3B} \textbf{77.03 ± 0.67}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} \textit{\textbf{64.23 ± 3.48}}}} & {\color[HTML]{3B3B3B} 63.7 ± 1.47} & {\color[HTML]{3B3B3B} 1575} \\ \hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{3B3B3B} Dev}} & {\color[HTML]{3B3B3B} \textbf{cases w/o SV}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 70.1 ± 7.44}} & {\color[HTML]{3B3B3B} \textbf{76.6 ± 1.08}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 74.67 ± 4.98}} & {\color[HTML]{3B3B3B} \textbf{80.63 ± 1.01}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 68.17 ± 1.72}} & {\color[HTML]{3B3B3B} \textbf{69.23 ± 0.7}} & 1338 \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/ SV}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 46.1 ± 6.24}} & {\color[HTML]{3B3B3B} \textbf{54.33 ± 1.1}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 54.03 ± 6.11}} & {\color[HTML]{3B3B3B} \textbf{64.6 ± 3.48}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 50.1 ± 3.7}} & {\color[HTML]{3B3B3B} \textbf{51.6 ± 1.99}} & 178 \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{all}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 67.23 ± 7.0}} & {\color[HTML]{3B3B3B} \textbf{74.33 ± 1.0}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 72.37 ± 5.01}} & {\color[HTML]{3B3B3B} \textbf{78.83 ± 1.27}} & \multicolumn{1}{c|}{{\color[HTML]{3B3B3B} 66.5 ± 2.19}} & {\color[HTML]{3B3B3B} \textbf{67.6 ± 0.56}} & 1516 \\ \hline

\multicolumn{1}{|c|}{LegalBERT} & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{mac}}} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{mic}}} & \multicolumn{2}{c|}{{\color[HTML]{3B3B3B} \textbf{hm}}} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|c|}{Test} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{normal} & soft & \multicolumn{1}{c|}{normal} & soft & \multicolumn{1}{c|}{normal} & soft & count \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/o SV}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 69.47 ± 1.69}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{72.17 ± 0.97}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 75.1 ± 0.56}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{78.97 ± 0.8}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{69.07 ± 1.8}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 67.03 ± 0.4}} & {\color[HTML]{3B3B3B} \textbf{1416}} \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/ SV}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{59.23 ± 3.98}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 56.37 ± 2.61}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 58.93 ± 1.4}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{59.47 ± 2.95}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{59.33 ± 3.93}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 52.27 ± 4.47}} & {\color[HTML]{3B3B3B} 159} \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{all}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 68.77 ± 1.16}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{70.53 ± 1.07}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 73.57 ± 0.6}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{77.1 ± 0.46}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{68.03 ± 1.29}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 65.17 ± 0.8}} & {\color[HTML]{3B3B3B} 1575} \\ \hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|c|}{{\color[HTML]{3B3B3B} Dev}} & {\color[HTML]{3B3B3B} \textbf{cases w/o SV}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 74.77 ± 1.65}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{75.67 ± 1.01}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 76.63 ± 0.76}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{80.1 ± 0.5}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{70.63 ± 0.64}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 69.87 ± 0.91}} & 1338 \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{cases w/ SV}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 45.83 ± 3.86}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{51.87 ± 1.39}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 53.77 ± 3.95}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{62.07 ± 1.15}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 50.37 ± 3.49}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{52.43 ± 4.4}}} & 178 \\ \hline
 & {\color[HTML]{3B3B3B} \textbf{all}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 71.6 ± 1.61}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{73.5 ± 0.44}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 74.1 ± 1.04}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{78.1 ± 0.36}}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} 68.3 ± 0.95}} & \multicolumn{1}{r|}{{\color[HTML]{3B3B3B} \textbf{68.3 ± 0.66}}} & 1516 \\ \hline
\end{tabular}
}


==> table/ue_results.tex <==
\resizebox{0.49\textwidth}{!}{


\begin{tabular}{|r|r|r|r|r|}
\hline
\multicolumn{1}{|l|}{} & \textbf{p value} & \textbf{t value} & \textbf{roc} & \textbf{pr} \\ \hline
\multicolumn{1}{|l|}{LegalBERT} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
entropy & \textbf{8.69E-03} & 2.63 & \textbf{0.59} & \textbf{0.09} \\ \hline
sr & \textbf{2.61E-02} & 2.23 & \textbf{0.59} & \textbf{0.09} \\ \hline
md & 3.32E-02 & -2.13 & 0.43 & 0.07 \\ \hline
ddu & 4.18E-07 & -5.08 & 0.36 & 0.05 \\ \hline

% \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{1}{|l|}{BERT} & \textbf{p value} & \textbf{t value} & \textbf{roc} & \textbf{pr} \\ \hline
entropy & \textbf{0.02} & 2.39 & 0.57 & 0.08 \\ \hline
sr & 0.08 & 1.75 & 0.57 & 0.08 \\ \hline
md & \textbf{7e-7} & 4.51 & \textbf{0.62} & \textbf{0.11} \\ \hline
ddu & 2e-7 & -4.76 & 0.38 & 0.05 \\ \hline
\multicolumn{1}{|l|}{Random} & 0.33 & 0.97 & 0.53 & 0.07 \\ \hline
\end{tabular}
}
% \begin{tabular}{|l|ccl|ccl|}
% \hline
%  & \multicolumn{3}{c|}{ROC AUC} & \multicolumn{3}{c|}{PR AUC} \\ \hline
%  & \multicolumn{1}{c|}{BERT} & \multicolumn{1}{c|}{LegalBERT} & \multicolumn{1}{c|}{random} & \multicolumn{1}{c|}{BERT} & \multicolumn{1}{c|}{LegalBERT} & \multicolumn{1}{c|}{random} \\ \hline
% Random & \multicolumn{1}{c|}{X} & \multicolumn{1}{c|}{X} &  & \multicolumn{1}{c|}{X} & \multicolumn{1}{c|}{X} &  \\ \hline
% Entropy & \multicolumn{1}{c|}{0.571} & \multicolumn{1}{c|}{0.566} &  & \multicolumn{1}{c|}{0.081} & \multicolumn{1}{c|}{0.092} &  \\ \hline
% MD & \multicolumn{1}{c|}{0.626} & \multicolumn{1}{c|}{0.639} &  & \multicolumn{1}{c|}{0.108} & \multicolumn{1}{c|}{0.103} &  \\ \hline
% RDE & \multicolumn{1}{c|}{0.502} & \multicolumn{1}{c|}{0.539} &  & \multicolumn{1}{c|}{0.066} & \multicolumn{1}{c|}{0.071} &  \\ \hline
% DDU & \multicolumn{1}{c|}{X} & \multicolumn{1}{c|}{X} &  & \multicolumn{1}{c|}{X} & \multicolumn{1}{c|}{X} &  \\ \hline
% HUD-MD & \multicolumn{1}{c|}{0.602} & \multicolumn{1}{c|}{0.619} &  & \multicolumn{1}{c|}{0.09} & \multicolumn{1}{c|}{0.103} &  \\ \hline
% HUD-RDE & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{0.538} &  & \multicolumn{1}{c|}{0.067} & \multicolumn{1}{c|}{0.085} &  \\ \hline
% HUD-DDU & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
% Decision Tree & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
% \end{tabular}


% }

==> text/depre_taxonomy.tex <==

++TODO++(Paraphrase needed) To encourage a principled and shared understanding of uncertainty in legal NLP, we provide a detailed account of uncertainty sources.
We characterise the main sources of uncertainty from a multi-disciplinary perspective by proposing the \enquote{Direction of Fit} of legal decision process, and a cirular taxonomy that is more informative and faithful than the popular aleatoric/epistemic dichotomy in privious works (Related Work).

\subsection{Legal and Linguistic Background} \label{sec:DoF}
++TODO++ Rewrite  

- Previous works used “\textbf{Triangle of Reference}” (Ogden and Richards, 1923, from XXX, Figure 1) to conceptualise the annotation process and build taxonomy of annotation disagreement (Aroyo \& Welty, 2015; Jiang \& Marneffen 2022); \\

- The “Triangle of Reference”-based models focuses on how linguistic symbols relate to the objects they represent. To explain the uncertainty sources in NLG tasks, Baan et al. 2023 extend it to the \textbf{“double triangle of language production}” (Figure 2), catering the more complex case of language production

- Legal scholar conceive the decision-making process in case-law of a \textbf{circular nature} (Figure 3, Oana Ichim) and consist of two directions: judges rule cases based on interpretation of existing normative structure/ case-law (Law-to-Case);  The output of the case decision/rulings at the same time serve as a basis for future litigation (Case-to-Law)

- To better reflect the decision-making process in case-law, we propose to use the "\textbf{Direction of Fit} (DoF)" framework (Figure 3) from speech act theory (Searle \& Vanderveken, (1985). “DoF” focuses on how language and intentions are related to the real world and how they guide our actions and interpretations of reality.

- Based on Figure 3 and Figure 4, we propose the DoF framework of decision making process in casa-law as shown in 


\subsection{Sources of Uncertainty in Case-law}

\noindent\textbf{Definition of Uncertainty} in this work: similar text desciprition of similar situation get differernt legal judgement. For example: ++TODO++ example (country difference: russian journalist vs. german journalist; vulnerable group: positive obligation to protect vulnerable individuals; temporal shift with the develop of the contry ):

\\
As discussed in \autoref{sec:DoF}, there are two direction of fit: Word-to-World Fit (blue) and  World-to-Word (red) / Case Document to Case Fact.

Ambiguitity comes from: this path is not one-to-one:
\textbf{(1) Same wording/phrase for the different realities: 
}\enquote{the self-referential wording of the ECtHR (Fikfak, 2021) - the court uses similar phrases in cases against the same respondent state or alleging the same violation, the model may learn that these are particularly relevant, even though this does not represent the legal reality. In this regard, it is questionable whether cases of the ECtHR can be considered “natural language”.}

\textbf{(2) Same norms for different situations} 
\enquote{Oana: in law where a general norm is applied to different situations.  Uncertainty is because we cannot account for the variety of situations in which that norm was applied. There are two questions here for instance: a) why positive obligations are applied to so many different situations and b) where they applied because the judges have not clearly defined positive obligations?}

\textbf{Echoed by Baan et al. 2023}, Section 3.1: \enquote{multiple possible worlds give rise to uncertainty. Variation in human language production, therefore, gives rise to uncertainty about a response given a context}






% \noindent\textbf{Taxonomy}\\
\\\subsection{Proxy Variables}\\



"there are many phenomena or sources that lead to uncertainty - "the same to different " mentioned above. A disentangled representation of these sources is crucial for trustworthy Legal NLP."

To quantitatively investigate how the agreement of judges’ decisions are influenced by different taxonomic categories, we derive proxy variables together with experts\\
\autoref{fig:taxonomy} offers an overview of the taxonomy of sources of uncertainty in legal decsion process in ECHR

\noindent\textbf{Fact $\rightarrow$ Decision}\\
\begin{itemize}
    \item Dissenting Opinion
    \item Split Vote
    \item Key case
\end{itemize}

\noindent\textbf{Decision $\rightarrow$ Fact}\\
\begin{itemize}
    \item Subject matter
    \item Defending country
    \item Categories of applicant (Vulnerability)
    \item Extent of control
\end{itemize}
\noindent\textbf{Longitudinal/Temporal}
\begin{itemize}
    \item Period / Social-political Context
    \item Remedies (Turn-over cases)
\end{itemize}
\noindent\textbf{ Association between SV and Proxies}\\
We assess statistical association between the proxy variables and whether a case is split-vote. 


\noindent \textbf{Results and Discussion}










==> text/ue.tex <==
PVI scores can’t represent the degree of judge’s agreement well can can be attributed to the fact the PVI measures predictive entropy which confounds epistemic and aleatoric uncertainty (cite DDU). In this section,  we disentangle aleatoric uncertainty (AU) and epistemic uncertainty (EU) to better investigate the uncertainty evaluation in COC. Epistemic (aka model) uncertainty refers to uncertainty caused by a lack of knowledge (about the best model), which can result from out-of-distribution examples. In theory, OOD inputs are should have higher epistemic Uncertainty as the the input data is extracted with the unknown subspace. Out-of-distribution (OOD)/outlier detection detection is a usual method to evaluate the quality of Epistemic uncertainty representation (cite Mukhoti, Vazhentsev, van Amersfoort).%https://arxiv.org/abs/2003.02037
On the opposite, AU refers to the variability in the outcome of an experiment which is due to inherently ambiguity. Following Vazhentsev, we define the cases with SV as ambiguous in-distribution (AID) - predictions which have higher values of aleatoric uncertainty. We use AID/ (SV cases) detection to evaluate the Aleatoric Uncertainty Estimation.

\noindent\textbf{Models}: Hierarchical BERT and LegalBERT finetuned on LexGlue A|B as mentioned in section X. Please note, we do not directly train model on the SV cases detection. What we want to explore is whether a model trained for COC can represent aleatoric uncertainty. 

\noindent\textbf{Uncertainty Estimation Methods} \\


\noindent\textit{(a) Quantifying Aleatoric Uncertainty}:we use two well-known methods based on probabilities from the output softmax layer of a neural network: entropy (Gal, 2016) and Softmax Response (SR, Geifman and El-Yaniv, 2017):
$$
U_{\mathrm{A}}^{\mathrm{Ent}}(\mathbf{x})=-\sum_{c \in C} p(y=c \mid \mathbf{x}) \log p(y=c \mid \mathbf{x}), 
$$

$$
& U_{\mathrm{A}}^{\mathrm{SR}}(\mathbf{x})=1-\max _{c \in C} p(y=c \mid \mathbf{x}) .
$$
Entropy and SR have been proposed also as measures of total uncertainty, aggregating the epistemic and aleatoric uncertainty (Malinin and Gales, 2018). As our data set contains no OOD data, we assume split- and unanimous voted cases should have similar epistemic uncertainty distributions. Thus, these methods can mostly reflect the aleatoric uncertainty (van Amersfoort et al., 2020; Mukhoti et al., 2023).

\noindent\textit{(b) Quantifying Epistemic Uncertainty}: “Recent works have proposed a variety of computationally efficient methods for quantifying epistemic uncertainty on the basis of fitting the probability density of latent instance representations.” In this work, we experiment with Mahalanobis Distance (MD, Lee et al., 2018) and Deep Deterministic Uncertainty (DDU, Mukhoti et al., 2023). We choose these two methods due to their frequent use in the literature  as well as their memory and computation efficiency (Vazhentse, zhang )\\ %Zhang, Dell, et al. "Uncertainty quantification for text classification." Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval. 2023.
\textbf{MD} estimates the epistemic uncertainty by measuring the distance between a test instance and the simulated distributions of the closest class. Lee et al. (2018b), for each class, fits a Gaussian centered in a class centroid {μc}c∈C with a covariance matrix Σ shared across classes. The highest class conditional probability density p(h(x) | y = c) determines the confidence of the prediction, and the uncertainty score is computed as the Mahalanobis distance between h(x) and the closest centroid: (++paraphrasing needed)
\begin{equation}
U_{\mathrm{E}}^{\mathrm{MD}}(\mathbf{x})=\min _{c \in C}\left(h(\mathbf{x})-\mu_c\right)^T \Sigma^{-1}\left(h(\mathbf{x})-\mu_c\right) .
\end{equation}
\\
\textbf{DDU} (Mukhoti et al., 2023) fits a Gaussian Mixture Model (GMM) p(h(x), y) with a single mixture component per class. The uncertainty score is the probability density of h(x) under the GMM:
\begin{equation}
U_{\mathrm{E}}^{\mathrm{DDU}}(\mathbf{x})=\sum_{c \in C} p(h(\mathbf{x}) \mid y=c) p(y=c)
\end{equation}\\
where $p(h(\mathbf{x}) \mid y=c) \sim \mathcal{N}\left(h(\mathbf{x}) \mid \mu_c, \Sigma_c\right)$ and $p(y=c)=\frac{1}{|\mathcal{D}|} \sum_{\left(\mathbf{x}_i, y_i\right) \in \mathcal{D}} \mathbf{1}\left[y_i=c\right]$.\\

%(Ambiguity Meets Uncertainty: Investigating Uncertainty Estimation for Word Sense Disambiguation)


% \subsection{Methods and Metrics}
% \noindent\textbf{Uncertainty Evaluation Scores}
% \begin{itemize}
%     \item Aleatoric: Entropy, SR
%     \item Epistemic: MD, GMM
%     % \item train external Feature-based decision tree (Jiang TACL 2021) to estimate uncertainty (TODO)
%     % \begin{itemize}
%     %     \item Use difference proxies: keycase, vulnerable group, defending country, etc.
% \end{itemize}

\begin{table}[t]
    \input{table/ue_results}
    \caption{UE results. ++TODO+ 3 random seeds; random baseline; DDU; PVI}
    \label{tab:ue_results}
\end{table}

\noindent\textbf{Uncertainty Evaluation Metrics}\\
We compute the mean of the uncertainty scores among the AiD split-voted samples and the rest searately. Then, we perform an independent t-test to compare the mean uncertainty scores between these two groups, assuming that aleatoric uncertainty will generally be higher on samples from the AiD cases.
We also compare uncertainty scores on the AiD  and the rest cases by measuring the area under the receiver-operator curve (AUROC) and under the precision-recall curve (AUPR), An ideal model should create very different distributions of confidence scores on split- and unanimous-voted cases, thus maximizing AUROC and AUPR. 

\\
\\
\noindent\textbf{Results \& Discussion}: \autoref{tab:ue_results} presents t-test  (p- and t-value) and AiD detection (AUROC and AUPR) performance of hierarchical LegalBERT and BERT. We make the following observations: (i) For legalBERT, Aleatoric Uncertainty measures Entropy and SR performs better in AiD detection (higher AUROC and AUPR scores) than pure epistemic uncertainty metrics MD and DDU. The AiD cases have a significantly higher scores in aleatoric metrics (t>0, p<0.05), while the epistemic metrics fail to capture this trend (t<0). (ii) For BERT, surprisingly the epistemic UE method MD outperforms the aleatoric methods. This effect might appear because the majority uncertainty of BERT model arises from epistemic uncertainty which arises from a lack of knowledge or data; than aleatoric uncertainty - the inherent ambiguity of instances. (iii) the overall AiD detection performance is very low, especially the AUPR scores, which is more sensitive in such an imbalanced dataset. Overall, our results show that in-domain pre training (LegalBERT) helps the model to have better inherent aleatoric uncertainty representation. However, there is a need for further investigation and more datasets on how to make models align its uncertainty better with humans.


% \begin{itemize}
%     \item Human Oracle: votes from the judges
%     \item Random: simulate random votes from 17 judges. ECHR court has max. 17 judges.
% \end{itemize}




